Recovering a Message from an Incomplete Set of Noisy Fragments

We consider the problem of communicating over a channel that breaks the message block into fragments of random lengths, shuffles them out of order, and deletes a random fraction of the fragments. Such a channel is motivated by applications in molecular data storage and forensics, and we refer to it as the torn-paper channel. We characterize the capacity of this channel under arbitrary fragment length distributions and deletion probabilities. Precisely, we show that the capacity is given by a closed-form expression that can be interpreted as F - A, where F is the coverage fraction ,i.e., the fraction of the input codeword that is covered by output fragments, and A is an alignment cost incurred due to the lack of ordering in the output fragments. We then consider a noisy version of the problem, where the fragments are corrupted by binary symmetric noise. We derive upper and lower bounds to the capacity, both of which can be seen as F - A expressions. These bounds match for specific choices of fragment length distributions, and they are approximately tight in cases where there are not too many short fragments.

==> BigPiecesNoNoisy.tex <==
\BigPiecesNoNoisy*
Consider Lemma~\ref{Lemma:ConcBoundCoverageNoisy}. Since $\gamma$ is a value we can choose, choose it to be $ (J/L)$.
% \iscomment{Is $A$ supposed to be $J$?}
Note that
\begin{align*}
    F_{d}\{\gamma\log{n}\} &=\frac{E\left[N_1\mathbf{1}_{\{\vec{X}_i \in \Y_{\geq (J/L)\log{n}}\}}\right]}{\ell_n}.
\end{align*}
Now define the event 
\begin{align*}
\mathcal{J} \triangleq \left\{\Co_{d}\{\gamma\log{n}\} > E\left[N_1\mathbf{1}_{\{\vec{X}_i \in \Y_{\geq (J/L)\log{n}}\}}\middle/\ell_n\right] + \delta\right\}.
\end{align*}
From the general version of Lemma~\ref{Lemma:ConcBoundCoverage}, $\Pr(\mathcal{J}) \to 0$ as $n \to \infty$. Therefore we can write
\begin{align*}
    &H(\Y_{\geq J}) + H(\vec Z_{\geq J})\\
    &\leq H(\Y_{\geq J}|\overline{\mathcal{J}}) + H(\Y_{\geq J}|\mathcal{J})\Pr(\mathcal{J}) + 1 \\
    &\leq H(\Y_{\geq J}|\overline{\mathcal{J}}) + 2n\Pr(\mathcal{J}) + 1 \\
    &\leq 2n\left(E\left[N_1\mathbf{1}_{\{\vec{X}_i \in \Y_{\geq g}\}}\middle]\right/\ell_n + \delta\right) + o(n) \\
    &\stackrel{(a)}{\leq} 2n\left(E\left[N_1\mathbf{1}_{\{N_1 \geq (J/L)\log{n}\}}\middle/\ell_n\right] + \delta\right) + o(n) \\
    &\stackrel{(b)}{\leq} 2n\left(\sqrt{E[N_1^2]\Pr(N_1 \geq (J/L)\log{n})}/\ell_n + \delta\right) + o(n) \\ 
    &\stackrel{(c)}{\leq} 2n\left(\sqrt{E[N_1^2]\ell_nL}/(\ell_n\sqrt{J\log{n}})\right) + \delta) + o(n) \\
    &\stackrel{(d)}{\leq} 2n\left(S\sqrt{L/J} + \delta\right) + o(n),
\end{align*}
for some finite $S$. $(a)$ is true because we include the deleted fragments. $(b)$ is due to Cauchy-Schwarz inequality. $(c)$ is due to Markov Inequality and $(d)$ is due to $E[N_1/\log{n}]$ and $E[(N_1/\log{n})^2]$ being finite and bounded. Therefore this implies
\begin{align*}
    \lim_{n \to \infty}\frac{H(\Y_{\geq J})}{n} \leq 2\left(S\sqrt{L/J} + \delta\right).
\end{align*}
\newpage

==> ConverseFixedLengths.tex <==
In order to prove the converse, we partition the set $\Y$ into a set of parallel channels with pieces of fixed lengths, as the output. 
It turns out that we can 
% \avcomment{we show that we can?}
% \adicomment{It's implicit in the fano's expansion followed by the independence bound}
treat these channels as independent systems and derive an upper bound on each channel.
More precisely, let 
\begin{align}
    \Y_r \triangleq \left\{\vec{X}_i\in\Y:N_i = \lceil r\log{n}\rceil \right\},
\end{align}
where $r \in [0,n]$ 
% \iscomment{shouldn't $r$ take any real value? if $r$ is forced to be integer we may not get all possible fragment lengths} \adicomment{Yes, used $:$ by mistake}
and $\lceil\cdot\rceil$ refers to the least integer function. In general for any $r_i,r_j$ such that $\lceil r_i\log{n}\rceil = \lceil r_j\log{n}\rceil$, $\Y_{r_i} = \Y_{r_j}$.  Now define $r_k := \min\{r:\lceil r\log{n}\rceil = k\}$, where $k$ is an integer. 
% where $r \in \Gamma:=\left\{\frac{1}{\log{n}},\frac{2}{\log{n}},\dots,\frac{n}{\log{n}}\right\}$.
%  Let $\Y_{\leq r} := \{\Y_{r_k}:r_k\leq r\}$ and $\Y_{\geq r} := \{\Y_{r_k}:r_k\geq r\}$
Then, by Fano's inequality, we have that any achievable rate $R$ must satisfy
\begin{align}\label{eq:Fano}
    R &\leq \lim_{n \to \infty} \frac{I(X^n;\Y)}{n} \leq \lim_{n \to \infty} \frac{H(\Y)}{n} \leq \lim_{n\to\infty}\sum_{k=1}^{n} \frac{H(\Y_{r_k})}{n}.
\end{align}

% Let $Z^n$ be a string of $0$'s and $1$' which represent whether a bit has been flipped in that position in $X^n$. Also recall that $T_2^n$ is the sequence of tearing locations on string $X^n$. $\vec{Z}_r$ is the ordered set of substrings of size $r\log{n}$ extracted from $Z^n$ based on tearing locations $T_2^n$. That is if there are two successive $1$'s such that $T_i = 1$ and $T_j = 1$ such that $j-(i+1) = r\log{n}$, then $Z_{i+1}^{j} \in\vec Z_r$. $\vec X_r$ is defined in a similar way.
We will now use the fact that $|\Y_r|$ concentrates around its mean to tackle \eqref{eq:Fano}.
To that end, we define the event
% \begin{align}
$B = \{\vec X_1 \in \Y\}$ 
% and % \nonumber \\
%% IS: We can define B' later
% $\tilde B \triangleq \{X_1 \in \Y'_{\tilde{d}}\}$
% \end{align}
and
% \iscomment{when will we need $B$? should it be $\tilde B$?}\adi{Aditya: I'll make it $\tilde B$. We use it in equations \eqref{eq:FirstSumChainRule}}
\begin{align}
    q_{r,n} &= \text{Pr}\left(N_1 = \lceil r\log{n}\rceil\right) \nonumber \\
    e_{r,n} &= \text{Pr}\left(B\,\middle|\,N_1 = \lceil r\log{n}\rceil\right).
\end{align}
% Note that $e_{k,n}$ can equivalently be expressed as $E\left[\mathbf{1}_{B}\middle|\frac{k-1}{L}\log{n} \leq N_1 < \frac{k}{L}\log{n}\right]$. 
Additionally, we define the event 
\aln{
\mathcal{E}_{r,n} =
\{||\Y_{r}|-nq_{r,n}e_{r,n}/\ell_n|>\epsilon_n n/\ell_n\}.
}
% We establish that $|\Y_k|$ concentrates  in the following lemma.
% %  where $(a)$ is because $H(\Y_{< 1}) = o(n)$. We can prove this as follows:
% %  \begin{align}
% % &\frac{H(\Y_{< 1})}{n} \stackrel{(a)}{\leq} \frac1n \log\binom{n + 2^A -1}{n} \leq \frac nn \log\left(\frac{n+2^A-1}{n}\right) \\
% %     &= \log\left(1+\left(\frac{2^A - 1}{n}\right)\right) \stackrel{(b)}{\leq} \frac{2^A}{n} = n^{\Bar{A} - 1} \to 0, 
% % \end{align}
% % as $n \to \infty$. Here $A = \bar{A}\log{n},\text{ } \bar{A}< 1$ and $(a)$ follows from the fact that $\log{(1+x)} \leq x, x \geq 0$

% We define the event
% % \begin{align}
% $B = \{\vec{X}_1 \in \Y\}$ 
% % and % \nonumber \\
% %% IS: We can define B' later
% % $\tilde B \triangleq \{X_1 \in \Y'_{\tilde{d}}\}$
% % \end{align}
% and
% % \iscomment{when will we need $B$? should it be $\tilde B$?}\adi{Aditya: I'll make it $\tilde B$. We use it in equations \eqref{eq:FirstSumChainRule}}
% \begin{align}
%     q_{r,n} &= \text{Pr}\left(N_1 = \lceil r\log{n}\rceil\right) \nonumber \\
%     e_{r,n} &= \text{Pr}\left(B\,\middle|\,N_1 = \lceil r\log{n\rceil}\right) \nonumber\\
%     \mathcal{E}_{r,n} &:= \left\{\middle||\Y_r|-nq_{r,n}e_{r,n}/\ell_n\middle|>\epsilon_n n/\ell_n\right\}.
% \end{align}
We establish that $|\Y_r|$ concentrates  in the following lemma.
\begin{lemma}\label{lemma:y_kconc}
% The number of pieces in $\Y_k$ satisfies
For $\epsilon_{r,n} > 0$ and n large enough,
% \begin{align}
%     \Pr & \left(\middle||\Y_k| - nq_{k,n}e_{k,n}/\ell_n\middle|\geq \epsilon n/\ell_n\right) \nonumber \\
%     & \quad \quad \quad \leq 2e^{-n\epsilon^2/2\ell_n} + 2e^{-\frac{8 \epsilon^2 \ell_n}{(1+2\epsilon)} n}
% \end{align}
\begin{align}
    \Pr(\mathcal{E}_{r,n}) \leq 2e^{-n\epsilon_{r,n}^2/(2\ell_{n})} + 2e^{-\frac{8 \epsilon_{r,n}^2 \ell_n}{(1+2\epsilon_{r,n})} n}.
\end{align}
% \iscomment{Lemma is stated in terms of $\epsilon_{r,n}$, but then we have $\epsilon_n$}
% \adicomment{Done}


% % \iscomment{is the $\ell_n$ dividing or multiplying?}\adi{Aditya: Dividing, I've changed it}
\end{lemma}
The proof of the lemma is in Appendix~\ref{app:Y_rConc}. We set $\epsilon_{r,n} = 1/\left(r^{5/2}\log^2{n}\right)$ to guarantee that, for a fixed $r$, as $n \to \infty$, $\epsilon_{r,n} \to 0$ and  $\Pr(\mathcal{E}_{r,n}) \to 0$. The reason we make this choice of epsilon will be clear at the end of the section.
% Now we can claim that given $\bar{\mathcal{E}}_{r,n}$,
% \begin{align}
%      |\Y_{r}| \leq M_{r} := \left(\epsilon_n +q_{r,n}e_{r,n}\right)\frac{n}{\ell_n}.
% \end{align}
% \iscomment{what is $\vec X_r$ and $\vec Z_r$?}
   We note that the total number of possible distinct sequences in $\Y_r$ is less than $2^{ r\log{n} +1 } = 2n^r$.
Now given $\overline{\mathcal{E}}_{k,n}$, 
\begin{align}
  |\Y_r| \leq  M_r \triangleq \left(\epsilon_{r,n} + q_{r,n}e_{r,n}\right)n/\ell_n.
\end{align}

Now  we upper bound the term $H(\Y_r)$ as
    % follows (by conditioning on the event $\mathcal{E}_{r,n}$)
\begin{align}\label{eq:EntropyExpansion}
   &H(\Y_r) \leq H(\Y_r,\mathbf{1}_{\mathcal{E}_{r,n}}) = H(\mathbf{1}_{\mathcal{E}_{r,n}}) + H(\Y_r|\mathbf{1}_{\mathcal{E}_{r,n}}) \nonumber\\ 
   &\leq H(\Pr(\mathcal{E}_{r,n})) + 2n\Pr(\mathcal{E}_{r,n}) + H(\Y_r|\bar{\mathcal{E}}_{r,n}) \nonumber \\
   &\stackrel{(a)}{=} H(\Y_r|\bar{\mathcal{E}}_{r,n}) + o(1).
\end{align}
% where $(a)$ is due to law of total probability.
% \iscomment{not exactly law of total probability. Instead of saying this just add one more step showing the chain rule properly}
% \adicomment{Done}
To see why $(a)$ holds, note that, from Lemma~\ref{app:Y_rConc} (for $n$ large enough)
% \iscomment{should $\ell_{r,n}$ be just $\ell_n$? and the $\epsilon_n$ be $\epsilon_{r,n}$?}
% \adicomment{Done}
$$2n \Pr(\mathcal{E}_{r,n}) \leq 4n\left(e^{-n\epsilon_{r,n}^2/(2\ell_{n})} + 2e^{-\frac{8 \epsilon_{r,n}^2 \ell_n}{(1+2\epsilon_{r,n})} n}\right) = o(1).$$

% \iscomment{explain second inequality in more detail}
% \iscomment{the $o(1)$ also needs more explanation. $\Pr(\mathcal{E}_{r,n})$ goes to zero (for fixed $r$), but how do we know $n \Pr(\mathcal{E}_{r,n})$ goes to zero?}
% \adicomment{Done}


Conditioned on $\overline{\mathcal{E}}_{r,n}$, we can view $\Y_{r}$ as a histogram of at most $M_r$ elements distributed across all possible sequences of size $\lceil r\log{n}\rceil$. We can then use this to upper bound the entropy, similar to the counting argument in \cite{TPCglobecom,TPCLP}. 
Precisely,
\begin{align}\label{eq:EntropyUpperBound1}
    H & (\Y_r|\overline{\mathcal{E}}_{r,n}) 
    % \nonumber \\
    % & 
    \leq \log\binom{2n^{r} + M_r -1}{M_r} \nonumber \\
    &\leq M_r\log\left(\frac{e(2n^{r} + M_r - 1)}{M_r}\right) \nonumber \\
    &= M_r(\log(2n^{r} + M_r - 1) + \log{e} -\log{M_r}) \nonumber \\
    &\stackrel{(a)}{=} M_r\left[\max\middle(r\log{n},\log{M_r}\middle)
    + \log{e} -\log{M_r} +  P\right] \nonumber \\
    &\stackrel{(b)}{=} M_r\left[\left(r\log{n} - \log{M_r}\right)^+ 
    % \hspace{-2mm}
    + \log{e} + P\right] \nonumber \\
    &\leq(1+o(1))M_r(r-1)^+\log{n},
    % &= M\log{n}\left[\left(\frac{k}{L} - \frac{\log{M}}{\log{n}}\right)^+ +      o(1)\right] \\
    % &\leq M\log{n}\left[\left(\frac{k}{L} - 1\right)^+ +  o(1)\right].
\end{align}
\iscomment{strictly speaking that shouldn't be true, because it says that, for $r < 1$, $H(\Y_r|\overline{\mathcal{E}}_{r,n}) = 0$, and that shouldn't be true, right? Maybe we need to write just $r$ instead of $(r-1)^+$ above?}
% \iscomment{maybe just write $(1+ o(1)) M_r(r-1)^+\log{n}$ above? that will make the argument on (28) a bit simpler too}
% \adicomment{Done}
% \iscomment{It's not immediately obvious that
% $\log(2n^{r} + M_r - 1) = 
% \max(r\log{n},\log{M_r}) + 
% \min(\log(2 + \frac{M_r-1}{n^{r}}),
%     \log(1 + \frac{2n^r-1}{M_r}))
% $.
% Please add a bit of explanation, or an additional step to (26).
% }
% \adicomment{Done.}
% \iscomment{should it be $o(M_r r \log n)$?}
% \adicomment{Since $r$ is a real number both should be okay right?}
% \iscomment{but why do you write $o(M_{r_k} r_k \log n)$ in the next line then?}
where 
\begin{align}
   P := \min\left(\log\middle(2 + \frac{M_r-1}{n^{r}}\middle),
    \log\middle(1 + \frac{2n^r-1}{M_r}\middle)\right).
\end{align}
To see why $(a)$ is true, notice that
\begin{align}
    &\log(2n^{r} + M_r - 1) = r\log{n} + \log{\left(2 + \frac{M_r-1}{n^r}\right)} = \log{M_r} + \log{\left(1 + \frac{2n^r -1}{M_r}\right)}\nonumber \\
    &= \max(r\log{n},\log{M_r}) + 
\min\left(\log\left(2 + \frac{M_r-1}{n^{r}}\right),
    \log\left(1 + \frac{2n^r-1}{M_r}\right)\right),
\end{align}
since if $a = b + c = d + e$, then $a = \max{(b,d)} + \min{(c,e)}.$
% \iscomment{explain (a) as it's not easy to verify}
Moreover we claim in step $(b)$ of \eqref{eq:EntropyUpperBound1} that $P = o(M_rr\log{n})$. To see this note that 
\begin{align}\label{eq:OrderOfM_rrlogn}
    M_r r \log{n} = \frac{n}{\ell_n}\left(\epsilon_{r,n} + q_{r,n}e_{r,n}\right)\times r \log{n} \geq \frac{n}{r^{3/2}\ell_n\log{n}}.
\end{align}
Now for $n$ large enough we have that
\begin{align}
    P &= \min\left(\log\middle(2 + \frac{M_r-1}{n^{r}}\middle),
    \log\middle(1 + \frac{2n^r-1}{M_r}\middle)\right) \nonumber\\ 
    &\leq \min\left(\log\middle(2 + \frac{M_r}{n^{r}}\middle),
    \log\middle(1 + \frac{2n^r}{M_r}\middle)\right) \nonumber \\ 
    &\leq \log\left(2 + \frac{M_r}{n^{r}}\right) = \log\left(2 + \frac{n^{1-r}}{\ell_n}\left(q_{r,n}e_{r,n} + \epsilon_{r,n}\right)\right)  \nonumber \\
    &\leq  \log\left(2+2n^{1-r}\right) = o\left(\frac{n}{r^{3/2}\ell_n\log{n}}\right) = o(M_rr\log{n}),
\end{align}
% \iscomment{penultimate equality is unclear. How is an $M_r$ appearing outside of the $\log$?}
% \adicomment{Added an intermediate expression to make it clear}
% \iscomment{I still don't understand. What happened to the min? It became equal to $\log(2+n^{1-r})$? Also, I don't follow why $\log(2+n^{1-r}) = o(n/(r^{3/2} \ell_n))$}
% \adicomment{For $r\leq 1$ the first term is the minimum for $n$ large enough. But i've changed it to an inequality since $\min(a,b)\leq a$. And $\lim_{n \to \infty} \frac{\log{(2 + 2n^{1-r}})}{\left(n/r^{3/2}\log{n}\right)}=0$}
if $r$ is less than 1. Similarly if $r$ is greater than $1$ then, for $n$ large enough, it an be shown that
\begin{align}
    P \leq \log\left(1 + 2rn^{r-1}\log^2{n}\right) = o\left(\frac{n}{r^{3/2}\ell_n\log{n}}\right) =  o(M_rr\log{n}).
\end{align}
% \iscomment{where did the $M_r$ come from?}
% \adicomment{Done}
% and similarly
% \begin{align}
%   &H(\vec Z_r|\vec X_r,\Y_r) \leq H(\Pr(\mathcal{E}_{r,n})) + 2n\Pr(\mathcal{E}_{r,n}) + H(\vec Z_r|\vec X_r,\Y_r,\bar{\mathcal{E}}_{r,n}) \nonumber \\
%   &= H(\vec Z_r|\vec X_r,\Y_r,\bar{\mathcal{E}}_{r,n}) + o(1),
% \end{align}
Therefore from  \eqref{eq:Fano} and \eqref{eq:EntropyExpansion} as
\begin{align}\label{eq:ConditionedFano}
& \frac1n\sum_{k=1}^nH(\Y_{r_k}) \leq \frac1n \sum_{k=\log{n}}^n (1+o(1))M_{r_k}\log{n}(r_k-1) \nonumber \\
&= \frac{1+o(1)}{n}\sum_{k=\log{n}}^n\frac{n}{\ell_n}(q_{r,k}e_{r,k}+\epsilon_{r,n})\log{n}(r_k-1)\nonumber \\
     &\leq  \frac{1+ o(1)}{\ell_n} \sum_{k=\log{n}}^n r_k\log{n}q_{r_k,n}e_{r_k,n} -  \frac{\log{n}(1+o(1))}{\ell_n}\sum_{k=\log{n}}^nq_{r_k,n}e_{r_k,n} \nonumber \\
     &+ \frac{1+o(1)}{\ell_n\log{n}}\sum_{k=\log{n}}^n \frac{1}{r_k^{3/2}} 
    \stackrel{(a)}{=} (1+o(1))\left(\frac{E\left[N_1\mathbf{1}_{\tilde B}\right]}{\ell_n} - \frac{E\left[\mathbf{1}_{\tilde B}\right]\log{n}}{\ell_n}\right) + \frac{D}{\sqrt{\log{n}}},
\end{align}
% \iscomment{show more steps for the first equality above, it's hard to follow}
% \adicomment{Done. I changed $\epsilon = 1/r^3\log{n}$ just realised that would be needed}
% \iscomment{the summation in the third line $\sum_{k=1}^n$ should be $\sum_{k=\log n}^n$ ?}
where $D$ is a finite number. To see $(a)$, note that the result of the first two terms is a consequence of the definitions of $q_{r,n}$ and $e_{r,n}$. Then note that we can rewrite the third term (since $r_k\log{n} = k$) as follows,
\begin{align}\label{eq:convergence}
    \sum_{k=\log{n}}^n\frac{1}{r_k^{3/2}} = \log^{3/2}{n}\sum_{k=\log{n}}^n \frac{1}{k^{3/2}} \leq D \log^{3/2}{n}.
\end{align}
Here the summation $\sum_{k=\log{n}}^n \frac{1}{k^{3/2}}$ is convergent since $k$ is the set of monotonically increasing natural numbers.
% \iscomment{Is this enough? What if $\lceil(r_k/r_1)\rceil^2$ is the same integer for several consecutive $k$s? I think you will  need to use the actual definition of $r_k$}
% \adicomment{Changed the argument. Also picked $\epsilon = 1/r^{5/2}\log{n}$ to make it work}
Therefore from \eqref{eq:Fano} we can say that
\begin{align}
    R &\leq \lim_{n\to\infty} \left(\frac{E\left[N_1\mathbf{1}_{\tilde B}\right]}{\ell_n} - \frac{E\left[\mathbf{1}_{\tilde B}\right]\log{n}}{\ell_n} + \frac{D}{\sqrt{\log{n}}}\right) \nonumber\\
    &= \Co_d\{\log{n}\} - \RC_d\{\log{n}\}.
\end{align}
This proves the converse of Theorem~\ref{thm:Main}.


% Notice that these entropy terms contend with each other in the following way: If $H(\Y_r)$ is small, it means that the ``distance'' between pieces in $\Y_r$ are very close. This implies that pieces in $\Y_r$ are indistinguishable. Therefore given $(\Y_r,\vec X_r)$, it is intuitively harder to compare pieces in $\Y_r$ to $\vec X_r$ to construct $\vec Z_r$, therefore increasing the value of $H(\vec Z_r|\vec X_r,\Y_r)$. Carefully using this tension lets us apply a non trivial upper bound on the sum of these entropies in a certain regime. This is summarised in the following lemma
% \begin{lemma}\label{lem:NoisyUpperBound}
% If $(1 - 2H(p) -2/r) > 0$ then,
% \begin{align}\label{eq:Yconditioning}
%     H(\Y_r|\bar{\mathcal{E}}_{r,n}) + H(\vec{Z}_r|\vec{X}_r,\Y_r,\bar{\mathcal{E}}_{r,n}) \leq M_r\lceil r\log{n}\rceil - M_r\log{M_r} + o( M_r\lceil r\log{n} \rceil),
% \end{align}
% else
% \begin{align}\label{eq:Zconditioning}
%     H(\Y_r|\bar{\mathcal{E}}_{r,n}) + H(\vec{Z}_r|\vec{X}_r,\Y_r,\bar{\mathcal{E}}_{r,n}) \leq M_r\lceil r\log{n}\rceil + o( M_r\lceil r\log{n} \rceil).
% \end{align}

% \end{lemma}

% Lemma~\ref{lem:NoisyUpperBound} is proved in the Appendix~\ref{app:NoisyUpperBound}. Following this lemma and equation \eqref{eq:ConditionedFano} we can say that
% \begin{align}
%     &I(X^n;\Y) \leq \sum_{k = \log{n}}^{\frac{2\log{n}}{1-2H(p)}}M_{r_k}\lceil r\log{n}\rceil + \sum_{k=\frac{2\log{n}}{1-2H(p)}}^{n}\left(M_{r_k}\lceil r_k\log{n}\rceil
%     - M_{r_k}\log{M_{r_k}}\right) + \sum_{\log{n}}^{n}o\left(M_{r_k}\lceil r\log{n}\rceil\right) \nonumber\\ 
%     &- H(p)\sum_{k=\log{n}}^{n}M_{r_k}\lceil r_k\log{n}\rceil + o(n)
%     \leq (1-H(p))\log{n}\sum_{k = \log{n}}^{\frac{2\log{n}}{1-2H(p)}}r_kM_{r_k} - \log{n}\sum_{k=\frac{2\log{n}}{1-2H(p)}}^{n}M_{r_k} + o(n) \nonumber \\
%     &+ \sum_{\log{n}}^{n}o\left(M_{r_k}\lceil r\log{n}\rceil\right) \stackrel{(a)}{=} n\left((1-H(p))\frac{E\left[N_1\mathbf{1}_{N_1\geq\log{n}}\right]}{\ell_n} - \frac{\log{n}}{\ell_n}E\left[\mathbf{1}_{N_1\geq\frac{2}{1-2H(p)}\log{n}}\right]\right) + o(n),
% \end{align}
% where $(a)$ holds true since if for some function $g(n)$ and $A_{k,n}$, if $\sum_{k = 1}^{g(n)} A_{k,n} = B(n)$, then $\sum_{k = 1}^{g(n)} o\left(A_{k,n}\right) = o\left(B(n)\right)$.
% We can therefore conclude that
% \begin{align}
%     R &\leq \lim_{n \to \infty} \frac{I(X^n;\Y)}{n} =  \lim_{n \to \infty} \left((1-H(p))\frac{E\left[N_1\mathbf{1}_{N_1\geq\log{n}}\right]}{\ell_n} - \frac{\log{n}}{\ell_n}E\left[\mathbf{1}_{N_1\geq\frac{2}{1-2H(p)}\log{n}}\right]\right), \nonumber \\
%     &= (1-H(p))\Co\{\log{n}\} - \RC\left\{\frac{2\log{n}}{1-2H(p)}\right\}.
% \end{align}

% \adicomment{Some potential splitting ideas: 1) $(1-p+H(p))$ bound: Maybe too loose 2) $1-p$ bound, how to though? 3) Linear upper bound for all, maybe too loose?}


% With a $\log{n}$ split we get upper bound
% \begin{align*}
%     \lim_{n \to \infty} \left((1-H(p))\frac{E\left[N_1\mathbf{1}_{N_1\geq\log{n}}\right]}{\ell_n} - \frac{\log{n}}{\ell_n}E\left[\mathbf{1}_{N_1\geq\frac{2}{1-2H(p)}\log{n}}\right]\right)
% \end{align*}
% If we can prove $\log{n}/(1-p)$, we get
% \begin{align*}
%     \lim_{n \to \infty} \left((1-H(p))\frac{E\left[N_1\mathbf{1}_{N_1\geq\frac{\log{n}}{1-H(p)}}\right]}{\ell_n} - \frac{\log{n}}{\ell_n}E\left[\mathbf{1}_{N_1\geq\frac{2}{1-2H(p)}\log{n}}\right]\right)
% \end{align*}




==> Defs.tex <==
% !TEX root = main.tex

\renewcommand{\L}{{\mathcal L}}

\newcommand{\1}{{\bf 1}}
\newcommand{\Z}{{\mathds Z}}
\newcommand{\dis}{{\mathsf{dis}} \,}
\newcommand{\ep}{\epsilon}
\newcommand{\vep}{\varepsilon}


\newcommand{\bA}{\mathsf{A}}
\newcommand{\bC}{\mathsf{C}}
\newcommand{\bG}{\mathsf{G}}
\newcommand{\bT}{\mathsf{T}}



\newcommand{\A}{{\mathcal A}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\C}{{\mathcal C}}

\newcommand{\G}{{\mathcal G}}
\renewcommand{\H}{{\mathcal H}}
\newcommand{\D}{{\mathcal D}}
%\newcommand{\Dr}{{\mathscr D}}

\newcommand{\Dr}{\mathcal{DR}}
%\newcommand{\dof}{\mathscr{D}}
\newcommand{\dof}{\mathbf{D}}
\newcommand{\Dreg}{\dof}


\newcommand{\E}{{\mathcal E}}
\newcommand{\V}{{\mathcal V}}
\renewcommand{\S}{{\mathcal S}}
\newcommand{\I}{{\mathcal I}}
\newcommand{\M}{{\mathcal M}}
\newcommand{\N}{{\mathcal N}}
\newcommand{\U}{{\mathcal U}}
\newcommand{\T}{{\mathcal T}}
\newcommand{\IN}{{\mathbb N}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Rs}{{\mathcal R}}
\newcommand{\Os}{{\mathcal O}}
\newcommand{\Ps}{{\mathcal P}}
\newcommand{\K}{{\mathcal K}}
\newcommand{\W}{{\mathcal W}}
\newcommand{\X}{{\mathcal X}}
\newcommand{\vX}{{\vec{X}}}
\newcommand{\Y}{{\mathcal Y}}
% \newcommand{\Z}{{\mathcal Z}}
\newcommand{\vY}{{\vec{Y}}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\dE}{D_\Sigma}
\newcommand{\q}[2]{Q_{s_{#1},d_{#2}}}
\newcommand{\p}[2]{P_{s_{#1},d_{#2}}}
\newcommand{\m}[2]{M_{s_{#1},d_{#2}}}
%\newcommand{\z}[2]{Z_{s_{#1},d_{#2}}}
\newcommand{\ttt}{3 \times 3 \times 3}
\newcommand{\kkk}{K \times K \times K}
\newcommand{\kk}[1]{#1 \times #1 \times #1}
\newcommand{\cT}{{\cal T}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cC}{{\cal C}}


\newcommand{\s}{{\bf s}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bc}{{\bf c}}

\newcommand{\EP}{{\rm EP}}

\newcommand{\setx}{\{ x_{(i)}^{K} \}_M }
\newcommand{\setxM}[1]{\{ x_{(i)}^{K} \}_{#1} }

\newcommand{\setX}{\{ X_{(i)}^{K} \}_M }
\newcommand{\setXM}[1]{\{ X_{(i)}^{K} \}_{#1} }

\newcommand{\sety}{\{ y_{(i)}^{K} \}_N }
\newcommand{\setyN}[1]{\{ y_{(i)}^{K} \}_{#1} }

\newcommand{\setY}{\{ Y_{(i)}^{K} \}_N }
\newcommand{\setYN}[1]{\{ Y_{(i)}^{K} \}_{#1} }

\newcommand{\bp}{{\bf p}}
\renewcommand{\r}{{\bf r}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\z}{{\bf z}}

\newcommand{\Cunc}{C_\text{unc}}






\newcommand{\aln}[1]{\begin{align*}#1\end{align*}}

\newcommand{\al}[1]{\begin{align}#1\end{align}}


\newcounter{numcount}
\setcounter{numcount}{1}

\newcommand{\eqnum}{\stackrel{(\roman{numcount})}{=}\stepcounter{numcount}}
\newcommand{\leqnum}{\stackrel{(\roman{numcount})}{\leq\;}\stepcounter{numcount}}
\newcommand{\geqnum}{\stackrel{(\roman{numcount})}{\geq\;}\stepcounter{numcount}}
\newcommand{\cnt}{$(\roman{numcount})$ \stepcounter{numcount}}
\newcommand{\rescnt}{\setcounter{numcount}{1}}


% \newcommand{\iscomment}[1]{{\color{blue} \bf{{{{IS --- #1}}}}}}    

% \newcommand{\cov}{{\rm \text{coverage}}}
% \newcommand{\recost}{{\rm \text{reordering~cost}}}

\newcommand{\Co}{{\rm C}}
\newcommand{\RC}{{\rm R}}


\newif\iflong
\longtrue

\newif\ifdraft
\drafttrue

\newcommand{\iscomment}[1]{
\ifdraft
{\color{blue} \bf{{{{IS --- #1}}}}}
\else
\fi
}    


\newcommand{\bluechange}[1]{{\leavevmode\color{blue}{#1}}}




==> NoisyUpperBound.tex <==
The key step to proving this lemma is employ Lemma~1 in \cite{noisyshuffling}, which evaluates the capacity of the noisy shuffling channel under certain conditions. Before proceeding we rewrite the lemma here (Let $\vec{\hat{X}}_r$ be define as $\vec{\hat{X}}_r := \vec X_r \oplus\vec Z_r$).

\begin{lemma}\label{lem:NoisyShuffling}
For a set $Y^{M_r}$, where $Y^{M_r}$ is an ordered random permutation of $\vec{\hat{X}}_r$, encoded by the uniformly distributed shuffle vector $S^{M_r} \in \{1:M_r\}^{M_r}$, if
\begin{align}
    1 - 2H(p) -\frac2r \geq 0,
\end{align}
then
\begin{align}
    H(Y^{M_r}) + H(S^{M_r}|\vec X_r,Y^{M_r}) \leq M_r(\lceil r\log{n}\rceil) + o(M_r(r\log{n})),
\end{align}
else we can show that 
\begin{align}
     H(Y^{M_r}) + H(S^{M_r}|\vec X_r,Y^{M_r}) \leq M_r(\lceil r\log{n}\rceil) + M_r\log{M_r} + o(M_r(r\log{n})).
\end{align}
\end{lemma}

Notice that Lemma~\ref{lem:NoisyShuffling} is very similar to Lemma~\ref{lem:NoisyUpperBound}. In essence to utilize this lemma, we convert quantities $\Y_r,\vec Z_r$ in terms of $Y^{M_r},S^{M_r}$. 
To do this we note that, given $\overline{\mathcal{E}}_{r,n}$, each parallel channel with output set $\Y_r$ is a noisy shuffling channel with atmost $M_r$ reads, which takes fixed size reads of size $r\log{n}$ as input, adds BSC$(p)$ noise to these reads and shuffles them. 
\adicomment{Can we claim this? It feels obvious to me, but I'm not sure how I'd want to explain it precisely}
We can view this output as either the unordered set $\Y_r$ or an ordered (but uniformly random) permutation $Y^{|Y_r|}$.
We thus note that $I(\vec{X}_r;\Y_r|\overline{\mathcal{E}}_{r,n}) = I(\vec{X}_r;Y^{|Y_r|}|\overline{\mathcal{E}}_{r,n})$. We can then expand the left hand side as follows
\begin{align}\label{eq:LHSChannelEquivalence}
    &I(\vec{X}_r;\Y_r|\overline{\mathcal{E}}_{r,n}) = H(\Y_r|\overline{\mathcal{E}}_{r,n}) - H(\Y_r|\vec X_r,\overline{\mathcal{E}}_{r,n}) \nonumber\\
    &= H(\Y_r|\overline{\mathcal{E}}_{r,n}) + H(\vec Z_r|\vec X_r,\Y_r,\overline{\mathcal{E}}_{r,n}) - H(\vec Z_r|\overline{\mathcal{E}}_{r,n}) -H(\Y_r|\vec X_r, \vec Z_r,\overline{\mathcal{E}}_{r,n}) \nonumber \\
    &\stackrel{(a)}{\geq}  H(\Y_r|\overline{\mathcal{E}}_{r,n}) + H(\vec Z_r|\vec X_r, \Y_r,\overline{\mathcal{E}}_{r,n}) - H(\vec Z_r|\overline{\mathcal{E}}_{r,n}),
\end{align}
where $(a)$ is because $|Y_r| \leq M_r$ and given $(\vec X_r, \vec Z_r)$, we can calculate $\Y_r$. Now following the steps in equation~(7,8) in \cite{noisyshuffling} we can argue that
\begin{align}\label{eq:RHSChannelEquivalence}
    &I(\vec{X}_r;Y^{|Y_r|}|\overline{\mathcal{E}}_{r,n}) = H(Y^{|Y_r|}|\overline{\mathcal{E}}_{r,n}) + H(S^{|Y_r|}|\vec{X}_r,Y^{|Y_r|},\overline{\mathcal{E}}_{r,n}) - H(S^{|Y_r|},\vec{Z}_r,Y^{|Y_r|}|\vec X_r,\overline{\mathcal{E}}_{r,n}) \nonumber \\
    &= H(Y^{|Y_r|}|\overline{\mathcal{E}}_{r,n}) + H(S^{|Y_r|}|\vec{X}_r,Y^{|Y_r|},\overline{\mathcal{E}}_{r,n}) - H(S^{|Y_r|}|\overline{\mathcal{E}}_{r,n}) - H(\vec{Z}_r|\overline{\mathcal{E}}_{r,n})\nonumber \\
    &\stackrel{(a)}{\leq} H(Y^{M_r}|\overline{\mathcal{E}}_{r,n}) + H(S^{M_r}|\vec{X}_r,Y^{M_r},\overline{\mathcal{E}}_{r,n}) - H(\vec Z_r|\overline{\mathcal{E}}_{r,n}) - \left(M_r-\frac{2n\epsilon_{r,n}}{\ell_n}\right)\log{\left(M_r-\frac{2n\epsilon_{r,n}}{\ell_n}\right)} \nonumber\\
    &= H(Y^{M_r}|\overline{\mathcal{E}}_{r,n}) + H(S^{M_r}|\vec{X}_r,Y^{M_r},\overline{\mathcal{E}}_{r,n}) - H(\vec Z_r|\overline{\mathcal{E}}_{r,n}) - \left(M_r-\frac{2n\epsilon_{r,n}}{\ell_n}\right)\log{\left(M_r-\frac{2n\epsilon_{r,n}}{\ell_n}\right)}
\end{align}
where $(a)$ because $H(S^{|Y_r|}) = |Y_r|\log{|Y_r|}$ and given $\overline{\mathcal{E}}_{r,n}$, $ |Y_r| \geq \frac{n}{\ell_n}(q_{r,n}e_{r,n} - \epsilon_n) = M_r - \frac{2n\epsilon_{r,n}}{\ell_n}$.


From \eqref{eq:LHSChannelEquivalence}, \eqref{eq:RHSChannelEquivalence} and Lemma~\ref{lem:NoisyShuffling} we can conclude that
\begin{align}
    H(\Y_r|\overline{\mathcal{E}}_{r,n}) + H(\vec Z_r|\vec X_r, \Y_r,\overline{\mathcal{E}}_{r,n}) \leq M_r(r\log{n})  - M_r\log{\left(M_r-\frac{2n\epsilon_{r,n}}{\ell_n}\right)} + o\left(M_rr\log{n}\right),
\end{align}
if $1-2H(p) - 2/r \geq 0$. Else if this condition is not satisfied then
\begin{align}
     &H(\Y_r|\overline{\mathcal{E}}_{r,n}) + H(\vec Z_r|\vec X_r, \Y_r,\overline{\mathcal{E}}_{r,n}) \leq M_r(r\log{n}) + M_r\log{M_r} - M_r\log{\left(M_r-\frac{2n\epsilon_{r,n}}{\ell_n}\right)} \nonumber \\
     &+  o( M_r(r\log{n})).
\end{align}
